Neural Network Quantization with AI Model Efficiency Toolkit (AIMET)

While neural networks have advanced the frontiers in many machine learning applications, they often come at a high computational cost. Reducing the power and latency of neural network inference is vital to integrating modern networks into edge devices with strict power and compute requirements. Neural network quantization is one of the most effective ways of achieving these savings, but the additional noise it induces can lead to accuracy degradation. In this white paper, we present an overview of neural network quantization using AI Model Efficiency Toolkit (AIMET). AIMET is a library of state-of-the-art quantization and compression algorithms designed to ease the effort required for model optimization and thus drive the broader AI ecosystem towards low latency and energy-efficient inference. AIMET provides users with the ability to simulate as well as optimize PyTorch and TensorFlow models. Specifically for quantization, AIMET includes various post-training quantization (PTQ, cf. chapter 4) and quantization-aware training (QAT, cf. chapter 5) techniques that guarantee near floating-point accuracy for 8-bit fixed-point inference. We provide a practical guide to quantization via AIMET by covering PTQ and QAT workflows, code examples and practical tips that enable users to efficiently and effectively quantize models using AIMET and reap the benefits of low-bit integer inference.

==> sections/amp.tex <==
\chapter{Automatic Mixed Precision (AMP)}
\section{Introduction}
\label{sec:amp}
\begin{itemize}
    \item [\colorbox{gray!40}{Description}]
    This technique helps choose per-layer integer bitwidths to retain model accuracy when run on fixed-point AI accelerators. For example, if a particular model is unable to meet a desired accuracy target when run on INT8 platform, Auto Mixed Precision feature shall find a minimal set of layers that need to run on other precision, say INT16, to get the desired accuracy. Choosing higher precision for some layers necessarily involves a trade-off: lower inferences/second for higher accuracy and vice-versa. The Auto Mixed Precision feature will generate a pareto curve that can guide the user to decide the right operating point for this tradeoff.
    For performing Auto Mixed Precision (AMP), the user needs create a Quantization Simulation model for a given model. This quant-sim model along with an allowable accuracy drop is passed to the auto mixed precision API. The function changes the Quantization simulation model in-place, to have different quantizers with different bitwidths. This simulation model can then be exported or evaluated to get a quantization accuracy.
   
    \begin{figure}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/AMP_sensitivity_analysis}
        \caption{Auto Mixed Precision example sensitivity list}
        \label{fig:amp_sensitivity_analysis}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/AMP_pareto_list}
        \caption{Auto Mixed Precision example pareto list}
        \label{fig:amp_pareto_list}            
    \end{figure}


    AIMET AMP algorithm involves three steps:
    \begin{enumerate}
        \item Find Layer Groups (Phase 0) : 
        Layer Groups are defined as a group of layers grouped together based on certain rules. This helps in reducing search space over which the mixed precision algorithm operates. It also ensures that we search only over the valid bitwidth settings for parameters and activations.        
        
        \item Perform Sensitivity Analysis (Phase 1) : 
        This will identify how sensitive is the model if we choose a lower quantization bitwidth for a particular layer group. The sensitivity analysis yields an accuracy list which is cached and can be re-used again by the algorithm.

        \item Create Pareto-Front list (Phase 2) : 
        Pareto curve is a trade-off curve that describes how accuracy varies given a BitOps target and vice versa. The AMP algorithm yields a pareto front curve which consists of Layer groups changed upto that point, relative bit ops (relative to starting bit ops), accuracy of the model and bitwidth to which the Layer group was changed to. An example of pareto list is as shown in figure~\ref{fig:amp_pareto_list}.
        The Pareto List can be used for plotting a pareto front curve.
    \end{enumerate}

    \item [\colorbox{gray!40}{API}]
    AIMET support one API to perform automatic mixed precision as shown below. A pareto\_front\_list is returned as output to the user.

    \begin{lstlisting}[caption={Automatic Mixed Precision},language=Python]
    from aimet_torch.pro.mixed_precision import choose_mixed_precision
    from aimet_torch.quantsim import QuantizationSimModel
    
    # Define parameters to pass to mixed precision algo
    dummy_input = torch.randn(1, 1, 28, 28).cuda()
    default_bitwidth = 16
    candidate_bitwidths = [(16, 16), (16, 8), (8, 16)]
    
    # Allowed accuracy drop in absolute value
    allowed_accuracy_drop = 0.5 # Implies 50% drop

    eval_callback_for_phase_1 = CallbackFunc(eval_callback_func, func_callback_args=5000)
    eval_callback_for_phase_2 = CallbackFunc(eval_callback_func, func_callback_args=None)

    forward_pass_call_back = CallbackFunc(forward_pass_callback, func_callback_args=dummy_input)

    # Create quantization simulation object
    sim = QuantizationSimModel(model, default_param_bw=default_bitwidth, default_output_bw=default_bitwidth,
                               dummy_input=dummy_input)
    sim.compute_encodings(forward_pass_callback, forward_pass_callback_args=None)

    # Apply automatic mixed precision algorithm with clean start = True 
    # i.e. new accuracy list and pareto list will be generated
    # If set to False then pareto front list and accuracy list will be loaded from the provided directory path
    pareto_front_list = choose_mixed_precision(sim, dummy_input, candidate_bitwidths,
                                               eval_callback_for_phase_1,
                                               eval_callback_for_phase_2,
                                               allowed_accuracy_drop,
                                               results_dir='./data',
                                               clean_start=True,
                                               forward_pass_callback=forward_pass_call_back)
    \end{lstlisting}

    \item [\colorbox{gray!40}{Usage Note}]   
        \item  A user can pass two different evaluation callbacks each for phase 1 and phase 2. Since phase 1 is measuring sensitivity of each quantizer group, we can pass a smaller representative dataset to phase 1 for evaluation. It is recommended to use complete dataset for evaluation in phase 2.
        \item There are two use-cases:
            \begin{enumerate}
                \item Choosing a very high accuracy drop (~1.0)- AIMET allows a user to save intermediate states for computation of pareto list. Therefore, if a user computes a pareto list corresponding to an accuracy drop ~1.0 they can view the complete profile of how model accuracy will vary as bit ops vary. Thereafter, user can visualize the pareto curve plot and choose an optimal point for accuracy. The algorithm can be re-run with the new accuracy drop to get a simulation model with the required accuracy. It must be noted here that the Pareto list is not modified during the second run.
                \item Choosing a lower accuracy drop and then continuing to compute pareto list from this point if more accuracy drop is acceptable. To enable this a user can use the clean\_start parameter in the API. If clean\_start is set to False then pareto list will start computation from the last point where it left off.
            \end{enumerate}
        \item It is recommended to use clean\_start parameter set to False to enforce usage of cached results for both the use cases.
        \item If the model or the candidate bitwidths change, it is recommneded that a clean start is performed by setting clean\_start to True.
\end{itemize}


==> tables/03_AdaRound_extensions.tex <==
\begin{table}[t]
    \centering
    \caption{Top-1 ImageNet validation accuracy (in $\%$) for W4A8 post-training per-tensor quantization with base and extended variants of AdaRound.}
    \label{tbl:04_adaround_extensions}
    \begin{tabular}{ l c c c c }
         Method & ResNet-18 & ResNet-50 &  InceptionV3 & MobileNetV2 \\
         \midrule       
         Full Precision & 69.68 & 76.07 & 77.40 & 71.72 \\
         \midrule  
         Nearest (W4A32) & 23.99 & 35.60 & 1.67 & 8.09 \\
         AdaRound & 
            68.48$\pm{}$0.08 & 
            74.96$\pm{}$0.05 & 
            75.66$\pm{}$0.12 & 
            69.21$\pm{}$0.07 \\ 
         + extensions & 
            \textbf{68.74}$\pm{}$\textbf{0.07} & 
            \textbf{75.21}$\pm{}$\textbf{0.11} &
            \textbf{75.87}$\pm{}$\textbf{0.05} & 
            \textbf{69.54}$\pm{}$\textbf{0.11} \\ 
    \end{tabular}
\end{table}


\begin{table}%1
\tabcolsep8pt
%\noautomaticrules
\tabletitle{Comparison of MATLAB and C Code for Simple Matrix Operations}%
\begin{tabular}{@{}lccc@{}}
\tch{Operations}    &\tch{Part of C Code} &\tch{Hor. fts.} &\tch{Ver. fts.}\\[-2pt]
Ball &19, 221 &4, 598   &3, 200\\
Pepsi$^a$&46, 281 &6, 898 &5, 400\\
Keybrd$^b$   &27, 290 &2, 968 &3, 405\\
Pepsi    &14, 796 &9, 188 &3, 209\\
\end{tabular}
\end{table}

==> tables/03_CLE.tex <==
\begin{table}[t]
     \centering
    \begin{tabular}{ l r r }
      \toprule
         Model          & FP32      & INT8 \\\midrule       % data act range est
         Original model & 71.72   &  0.12 \\            % 0.09
        %  Replace ReLU6  & 71.70\%   &  0.11\% \\            % 0.09
         + CLE    & 71.70   & 69.91 \\            % 69.61
         + absorbing bias & 71.57   & \textbf{70.92}  \\   % 70.49
         \midrule
         Per-channel quantization & 71.72 & 70.65 \\
         \bottomrule
          \end{tabular}
           \caption{Impact of cross-layer equalization (CLE) for \mnv{2}. ImageNet validation accuracy (\%), evaluated at full precision and 8-bit quantization.}
          \label{tbl:cle_mnv2}
\end{table}



==> tables/03_CLE_ShuffleNetV2.tex <==
\begin{table}[t]
    \centering
    \caption{Top-1 ImageNet validation accuracy (in $\%$) for ShuffleNetV2, evaluated at full precision and 8-bit integer quantized.}
     \label{tbl:04_cle_shufflenetv2}
    \begin{tabular}{ l r r }
         ShuffleNetV2          & \tt{x1.0}      & \tt{x0.5} \\
         \midrule       
         FP32 & 69.45 & 60.55 \\
         \midrule  
         Per-tensor quantization &  65.50 & 56.40 \\
         + DFQ   & 68.81   &  58.92  \\ 
         + CLE across blocks   & 68.92   &  \textbf{59.90}  \\ 
         \midrule
         Per-channel quantization & \textbf{69.00} & 59.87 \\
    \end{tabular}   
\end{table}


==> tables/03_adaround_ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ l c c }
        \toprule
         \qquad\qquad\quad Rounding          & First layer      & All layers \\\midrule
         Nearest            &  52.29   &  23.99 \\
         %H+G task loss (cf. \eqref{eq:taylor_opt0}) & 68.07$\pm$0.28    &  N/A \\
         $\mati{H}{\vec{w}}$ task loss (equation~\ref{eq:adaround_taylor}) & 68.62   &  N/A \\
         Cont.~relaxation MSE (equation~\ref{eq:adaround_relaxopt}) &  69.58   &  66.56 \\
         AdaRound (equation~\ref{eq:adaround_asym})     &  \textbf{69.58}   &  \textbf{68.60} \\
         \bottomrule
    \end{tabular}
\caption{Impact of various approximations and assumptions made in section~\ref{sec:adaround} on the ImageNet validation accuracy (\%) for~\rn{18} averaged over 5 runs. N/A implies that the corresponding experiment was computationally infeasible.}
\label{tab:adaround_ablation}
\end{table}

==> tables/03_adaround_deeplab_aimet.tex <==
\begin{table}[t]
    \centering
    \caption{AdaRound on DeepLabv3 Semantic Segmentation.}
    \label{tbl:adaround_deeplab_aimet}
    \begin{tabular}{ l c }
    \toprule
         Configuration & mIOU (Mean Intersection over Union)\\
    \midrule
     FP32 & 72.94\% \\
     Nearest Rounding (W4A8)  & 6.09\% \\
     AdaRound (W4A8)& 70.86\% \\
    \bottomrule
    \end{tabular}
\end{table}


==> tables/03_adaround_intro.tex <==
\begin{table}[t]
    \centering
     \caption{Comparison of ImageNet validation accuracy between rounding-to-nearest vs 100 stochastic rounding choices. We report the mean and the standard deviation of 100 stochastic \cite{Gupta2015} rounding choices (Stochastic) as well as the best validation performance among these samples (Stochastic (best)).}
       \label{tab:adaround_introtable}
    \begin{tabular}{ l r }
         Rounding scheme          & Acc(\%)       \\\midrule
         Nearest            & 52.29  \\
         Stochastic         & 52.06$\pm$5.52   \\ 
         Stochastic (best)  & 63.06  \\
    \end{tabular}
\end{table}

==> tables/03_bias_correction.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l r r}
    \toprule
        Model & FP32 & INT8\\\midrule
        Original Model          & 71.72           & 0.12\\  
        + bias correction               & 71.72           & \textbf{52.02}\\ \midrule
        CLE + bias absorption & 71.57           & 70.92\\   
        + bias correction   & 71.57           & \textbf{71.19}\\ 
     \bottomrule
    \end{tabular}
        \caption{Impact of bias correction for \mnv{2}. ImageNet validation accuracy (\%) evaluated at full precision and 8-bit quantization.}
     \label{tbl:04_bias_correction}
\end{table}


==> tables/03_range_setting_activations.tex <==
\begin{table*}[t]
    \centering
     \tabletitle{Top-1 ImageNet validation accuracy (\%) for different methods of range setting of activation (symmetric uniform) quantizers while keeping the weights in FP32.}
     \label{tab:rangesetting_activations}
    \begin{tabular}{ l | r r r | r r r}
        Model (FP32 val accuracy) & \multicolumn{3}{c|}{\rn{18} (69.68\%)} & \multicolumn{3}{c}{\mnv{2} (71.72\%)} \\ \midrule
         Method/Bit-width           & 8    & 6      & 4    & 8 & 6    & 4 \\\midrule
         Min-Max         & 69.60$\pm$0.03         &       67.85$\pm$0.13   & 13.50$\pm$1.92   & 70.97$\pm$0.07         &  63.17$\pm$0.98  & 0.33$\pm$0.05\\
         MSE          & 69.44$\pm$0.10         & 64.09$\pm$1.05         & 15.06$\pm$1.55     & 71.15$\pm$0.16         &  63.85$\pm$1.60  & 8.08$\pm$0.13\\
         MSE + Xent         & 69.57$\pm$0.08         & 68.66$\pm$0.09         & 55.78$\pm$0.63     & 71.35$\pm$0.04         &  68.48$\pm$0.20  & 30.09$\pm$1.06\\
         BN ($\alpha=6$)& 69.63         & 68.17 & 18.29     & 71.2         &  64.82  & 0.50\\
    \end{tabular}
\end{table*} 

==> tables/03_range_setting_activations_asym.tex <==
\begin{table*}[t]
    \centering

    \begin{tabular}{ l | r r r | r r r}
     \toprule
        Model (FP32 accuracy) & \multicolumn{3}{c|}{\rn{18} (69.68)} & \multicolumn{3}{c}{\mnv{2} (71.72)} \\ \midrule
         Bit-width        & \multicolumn{1}{c}{A8}    & \multicolumn{1}{c}{A6}      & \multicolumn{1}{c|}{A4}    & \multicolumn{1}{c}{A8} & \multicolumn{1}{c}{A6}    & \multicolumn{1}{c}{A4} \\\midrule
        %  Min-Max         & 69.60         &       68.49   & 23.54   & 70.94         &  62.99  & 0.5\\
        %  MSE          & 69.60         & 67.95        & 37.53     & 71.31         &  67.95  & 12.36\\
        %  MSE + Xent         & 69.59         & 68.91         & 59.62     & 71.35         &  68.83  & 29.81\\
        %  BN ($\alpha=6$)& 69.66         & 68.77 & 23.67     & 71.31         &  65.17  & 0.63\\
Min-Max     & 69.60 & 68.19 & 18.82 &	 70.96 & 64.58 & 0.53 \\
MSE         & 69.59 & 67.84 & 31.40 &	 71.35 & 67.55 & 13.57 \\
MSE + Xent  & \textbf{69.60} & \textbf{68.91} & \textbf{59.07} &	\textbf{71.36} & \textbf{68.85 }& \textbf{30.94} \\
BN ($\alpha=6$) & 69.54 & 68.73 & 23.83 &	 71.32 & 65.20 & 0.66 \\
\bottomrule
    \end{tabular}
 \caption{Ablation study for different methods of range setting of (asymmetric uniform) activation quantizers while keeping the weights in FP32. Average ImageNet validation accuracy (\%) over 5 runs.}
\label{tab:rangesetting_activations}
\end{table*} 

% Run commands for this table:
% python experiment_manager/scipts/white_paper/image_net_ptq.py tbl2-range-setting-activations --no-use-cluster --num-runs 5
% python experiment_manager/scipts/white_paper/image_net_ptq.py tbl2-range-setting-activations --no-use-cluster --num-runs 5 --architecture mobilenet_v2_cirqus_quantized

% Final validation top_1_accuracy Results (5 runs) in format: Mean (+-STD) [Best]:
% Opt1 / Opt2                                       |     --n-bits-act 8  |  --n-bits-act 6  |  --n-bits-act 4
% --act-quant-method running_minmax                 |     69.61 (+-0.01) .....    |       67.68 (+-0.19) .....    |       11.01 (+-1.27) .....
% --act-quant-method MSE                            |     69.59 (+-0.04) .....    |       67.70 (+-0.20) .....    |       34.30 (+-3.59) .....
% --act-quant-method MSE --cross-entropy-layer fc   |     69.59 (+-0.04) .....    |       67.70 (+-0.20) .....    |       34.30 (+-3.59) .....
% --act-quant-method BN_std_dev --std-dev 6         |     69.63 (+-0.02) .....    |       68.73 (+-0.05) .....    |       23.20 (+-0.18) .....

% Old one with error margins
% \begin{table*}[t]
%     % \centering
%      \tabletitle{Top1 ImageNet validation accuracy (\%) for different methods of range setting of activation (asymmetric uniform) quantizers while keeping the weights in FP32.}
%     \begin{tabular}{ l | r r r | r r r}
%         Model (FP32 acc.) & \multicolumn{3}{c|}{\rn{18} (69.68\%)} & \multicolumn{3}{c}{\mnv{2} (71.72\%)} \\ \midrule
%          Method/Bit-width           & 8    & 6      & 4    & 8 & 6    & 4 \\\midrule
%          Min-Max         & 69.60$\pm$0.05         &       68.49$\pm$0.07   & 23.54$\pm$3.85   & 70.94$\pm$0.1         &  62.99$\pm$1.31  & 0.5$\pm$0.15\\
%          MSE          & 69.60$\pm$0.03         & 67.95$\pm$0.28         & 37.53$\pm$7.35     & 71.31$\pm$0.05         &  67.95$\pm$0.84  & 12.36$\pm$0.47\\
%          MSE + Xent         & 69.59$\pm$0.07         & 68.91$\pm$0.09         & 59.62$\pm$0.52     & 71.35$\pm$0.02         &  68.83$\pm$0.0.08  & 29.81$\pm$1.54\\
%          BN ($\alpha=6$)& 69.66         & 68.77 & 23.67     & 71.31         &  65.17  & 0.63\\
%     \end{tabular}
%     \label{tab:rangesetting_activations}
% \end{table*} 

==> tables/03_range_setting_weights.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ l | r r r | r r r}
    \toprule
        Model (FP32 accuracy) & \multicolumn{3}{c|}{\rn{18} (69.68)} & \multicolumn{3}{c}{\mnv{2} (71.72)} \\ \midrule
        Bit-width        & \multicolumn{1}{c}{W8}    & \multicolumn{1}{c}{W6}      & \multicolumn{1}{c|}{W4}    & \multicolumn{1}{c}{W8} & \multicolumn{1}{c}{W6}    & \multicolumn{1}{c}{W4} \\\midrule
        %  Min-Max         & 69.49         & 66.27         & 0.41     & 71.52         &  69.64  & 18.16\\
        %  MSE         & 69.59         & 66.99         & 39.80     & 71.43         &  70.13  & 46.50 \\
        % \midrule
        %  Min-Max (Per-channel)         & 69.62         & 69.58         & 55.89     & 71.55         &  70.54  & 55.62\\
        %  MSE (Per-channel)        & 69.63         & 69.48         & 61.04     & 71.51        &  70.96  & 63.55 \\
Min-Max                 & \textbf{69.57} &	63.90 &	0.12 &	\textbf{71.16} &	64.48 &	0.59 \\
MSE                     & 69.45 &	\textbf{64.64} &	\textbf{18.82} &	71.15 &	\textbf{65.43} &	\textbf{13.77} \\ \midrule
Min-Max (Per-channel)   &69.60 &	69.08 &	44.49 &	71.21 &	68.52 &	18.40 \\
MSE (Per-channel)       &\textbf{69.66} &	\textbf{69.24} &	\textbf{54.67} &	\textbf{71.46} &	\textbf{68.89} &	\textbf{27.17} \\
\bottomrule
    \end{tabular}
\caption{Ablation study for different methods of range setting of (symmetric uniform) weight quantizers while keeping the activations in FP32. Average ImageNet validation accuracy (\%) over 5 runs.}
 \label{tab:rangesetting_weights}
\end{table*}



% Run commands for this table:
% python experiment_manager/scipts/white_paper/image_net_ptq.py tbl1-range-setting-weights --no-use-cluster --num-runs 5
% python experiment_manager/scipts/white_paper/image_net_ptq.py tbl1-range-setting-weights --no-use-cluster --num-runs 5 --architecture mobilenet_v2_cirqus_quantized

% Final validation top_1_accuracy Results (5 runs) in format: Mean (+-STD) [Best]:
% Opt1 / Opt2                                          |  --n-bits 8  |  --n-bits 6  |  --n-bits 4
% --weight-quant-method current_minmax                 |  69.57 (+-0.00) .....    |       63.90 (+-0.00) .....    |       0.12 (+-0.00) .....
% --weight-quant-method MSE                            |  69.45 (+-0.00) .....    |       64.64 (+-0.00) .....    |       18.82 (+-0.00) .....
% --weight-quant-method current_minmax --per-channel   |  69.60 (+-0.00) .....    |       69.08 (+-0.00) .....    |       44.49 (+-0.00) .....
% --weight-quant-method MSE --per-channel              |  69.66 (+-0.00) .....    |       69.24 (+-0.00) .....    |       54.67 (+-0.00) .....

==> tables/03_standard_ptq.tex <==

\begin{table*}[ht]
    \centering
    \begin{tabular}{ l | r| r r |  r r}
    \toprule
                         &       & \multicolumn{2}{c|}{Per-tensor} &
                         \multicolumn{2}{c}{Per-channel} \\ 
        %  \cmidrule(lr){3-4}   \cmidrule(lr){5-6}
        Models        & FP32  & W8A8    & W4A8      & W8A8    & W4A8 \\
        \midrule
\rn{18}	        & 69.68 & 69.60 & 68.62 & 69.56 & 68.91 \\
\rn{50}	        & 76.07 & 75.87 & 75.15 & 75.88 & 75.43 \\
\mnv{2}	        & 71.72 & 70.99 & 69.21 & 71.16 & 69.79 \\
InceptionV3	    & 77.40 & 77.68 & 76.48 & 77.71 & 76.82 \\
EfficientNet lite   & 75.42 & 75.25 & 71.24 & 75.39 & 74.01 \\
DeeplabV3	        & 72.94 & 72.44 & 70.80 & 72.27 & 71.67 \\
EfficientDet-D1	    & 40.08 & 38.29 & 0.31 & 38.67 & 35.08\\
BERT-base\textsuperscript{\dag} & 83.06 & 82.43 & 81.76 & 82.77 & 82.02 \\
\bottomrule
\end{tabular}
 \caption{Performance (average over 5 runs) of our standard PTQ pipeline for various models and tasks. DeeplabV3 (MobileNetV2 backbone) is evaluated on Pascal VOC (mean intersection over union), EfficientDet-D1 on COCO 2017 (mean average precision), BERT-base on the GLUE benchmark and other models on ImageNet (accuracy). We evaluate all models on the respective validation sets. Higher is better in all cases.~\textsuperscript{\dag}A few quantized activations are kept in higher precision (16 bits).}
 \label{tbl:standard_ptq}
\end{table*}

% Note on the numbers
% * W4A8 are all from the paper
% * EfficientNet from the efficientnet slide deck
% * Per-channel results from AdaRound slide deck


==> tables/04_bn_ablation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ l | r r | r r}
    \toprule
        Model (FP32 accuracy)                   & \multicolumn{2}{c|}{\rn{18} (69.68)} & \multicolumn{2}{c}{\mnv{2} (71.72)} \\ 
        \midrule
        Bit-width                           & W4A8  & W4A4   & W4A8   & W4A4 \\\midrule
        Static folding BN                   & \textbf{69.76} & \textbf{68.32}  & \textbf{70.17}  & \textbf{66.43} \\
        Double forward~\citep{krishnamoorthi} & 69.42 & 68.20  & 66.87  & 63.54 \\ \midrule
        Static folding (per-channel)        & 69.58 & 68.15  & \textbf{70.52}  & 66.32 \\ 
        Keep original BN (per-channel)      & \textbf{70.01} & \textbf{68.83}  & 70.48  & \textbf{66.89} \\
        \bottomrule
    \end{tabular}
     \caption{Ablation study with various ways to include BN into QAT. The learning rate is individually optimized for each configuration. Average ImageNet validation accuracy (\%) over 3 runs.}
     \label{tbl:bn_ablation}
\end{table*}


==> tables/04_cle_ablation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ l | r r | r r}
    \toprule
        Model (FP32 accuracy)                   & \multicolumn{2}{c|}{\rn{18} (69.68)} & \multicolumn{2}{c}{\mnv{2} (71.72)} \\ 
                                            & PTQ   & QAT    &  PTQ   & QAT \\ \midrule
        W4A8 baseline                       &  18.58 & 69.74  & 0.10 & 0.10 \\ %TODO check
        W4A8 w/ CLE                         &  16.29 & \textbf{69.76}  & 12.99 & \textbf{70.13} \\ 
        W4A8 w/ CLE + BC                    & 38.58  &  69.72 & 46.90 & 70.07 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study with various PTQ initialization. The learning rate is individually optimized for each configuration. ImageNet validation accuracy (\%) averaged over 3 runs.}
     \label{tbl:cle_init_ablation}
\end{table*}

%TODO update PTQ numbers

==> tables/04_quant_init_ablation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ l | r r | r r}
    \toprule
        Model (FP32 accuracy)                   & \multicolumn{2}{c|}{\rn{18} (69.68)} & \multicolumn{2}{c}{\mnv{2} (71.72)} \\ 
        % \cmidrule(lr){2-3}\cmidrule(lr){4-5}
                                            & PTQ   & QAT    &  PTQ   & QAT \\ \midrule
        W4A8 w/ min-max weight init         &  0.12 &  69.61 & 0.56 & 69.96  \\
        W4A8 w/ MSE weight init             &  18.58 &  \textbf{69.76} & 12.99 & \textbf{70.13}  \\ \midrule
        W4A4 w/ min-max act init            &  7.51 & 68.23 & 0.22 & \textbf{66.55} \\ 
        W4A4 w/ MSE  act init               &  9.62 & \textbf{68.41} & 0.71 & 66.29 \\ 
        \bottomrule
    \end{tabular}
     \caption{Ablation study for various ways to initialize the quantization grid. The learning rate is individually optimized for each configuration. ImageNet validation accuracy (\%) averaged over 3 runs.}
 \label{tbl:quant_init_ablation}
\end{table*}


==> tables/04_standard_qat.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ l | r| r r r |  r r r}
    \toprule
                         &       & \multicolumn{3}{c|}{Per-tensor} & \multicolumn{3}{c}{Per-channel} \\ 
        Models        & FP32  & W8A8    & W4A8      & W4A4  &  W8A8    & W4A8      & W4A4 \\
        \midrule
         \rn{18}         & 69.68 & 70.38   & 69.76  & 68.32  & 70.43  & 70.01  & 68.83 \\
        \rn{50}         & 76.07 & 76.21   & 75.89   & 75.10   & 76.58   & 76.52   & 75.53      \\
        InceptionV3	        & 77.40 & 78.33 & 77.84 & 77.49 & 78.45 & 78.12 & 77.74 \\
        \mnv{2}      & 71.72 & 71.76   & 70.17  & 66.43  & 71.82   & 70.48  & 66.89  \\ 
        EfficientNet lite   & 75.42 & 75.17 & 71.55 & 70.22 & 74.75 & 73.92 & 71.55 \\
        DeeplabV3	        & 72.94 & 73.99 & 70.90 & 66.78 & 72.87 & 73.01 & 68.90 \\
        EfficientDet-D1	 & 40.08   & 38.94    & 35.34 & 24.70    & 38.97   &  36.75   &  28.68 \\
        BERT-base &  83.06  & 83.26  & 82.64  & 78.83 & 82.44  & 82.39  & 77.63\\
        \bottomrule
    \end{tabular}
     \caption{Performance (average over 3 runs) of our standard QAT pipeline for various models and tasks. DeeplabV3 (\mnv{2} backbone) is evaluated on Pascal VOC (mean intersection over union), EfficientDet-D1 on COCO 2017 (mean average precision), BERT-base on the GLUE benchmark and all other models on ImageNet (accuracy). We evaluate all models on the respective validation sets. Higher is better in all cases.}
     \label{tbl:standard_qat}
\end{table*}

